Deep learning detects uncataloged low-frequency earthquakes across regions

Documenting the interplay between slow deformation and seismic ruptures is essential to understand the physics of earthquakes nucleation. However, slow deformation is often difficult to detect and characterize. The most pervasive seismic markers of slow slip are low-frequency earthquakes (LFEs) that allow resolving deformations at minute-scale. Detecting LFEs is hard, due to their emergent onsets and low signal-to-noise ratios, usually requiring region-specific template matching approaches. These approaches suffer from low flexibility and might miss LFEs as they are constrained to sources identified a priori. Here, we develop a deep learning-based workflow for LFE detection, modeled after classical earthquake detection with phase picking, phase association, and location. Across three regions with known LFE activity, we detect LFEs from both previously cataloged sources and newly identified sources. Furthermore, the approach is transferable across regions, enabling systematic studies of LFEs in regions without known LFE activity.

==> tables/workflow_params.tex <==
\begin{table}[ht!]
\caption{Parameters for the LFE detection workflow. The parameters are grouped into the velocity model, picking parameters, and association parameters. Parameter names follow the naming in the underlying tools SeisBench and PyOcto.\\}
\label{tab:workflow_params}
\centering
\begin{tabular}{lllll}
\toprule
Parameter & Cascadia & Guerrero & Nankai & San Andreas \\
\midrule
Velocity model & \cite{bostockMagnitudesMomentdurationScaling2015} & \cite{dominguez2006seismic} & JMA2001 & \cite{small2017scec} \\
\midrule
P\_threshold & 0.1 & 0.1 & 0.15 & 0.1 \\
S\_threshold & 0.1 & 0.1 & 0.15 & 0.1 \\
overlap & 600 & 600 & 600 & 600 \\
\midrule
minimum number picks & 13 & 14 & 12 & 10 \\
minimum number p and s picks & 2 & 3 & 3 & 2 \\
maximum std nonlinloc & 0.2 & 0.4 & 0.4 & 0.25 \\
pick match tolerance & 2.5 & 2.0 & 2.0 & 2.0 \\
velocity model tolerance & 2.0 & 2.0 & 2.0 & 2.0 \\
association cutoff distance & - & - & 150 & - \\
min pick fraction & 0.25 & 0.25 & 0.4 & 0.25 \\
\bottomrule
\end{tabular}
\end{table}

